LLM-Augmented Agent-Based Simulation of Cyber Social Agents

Social media bots are often portrayed as malicious automations to be detected and removed, but automation on social media platforms encompasses a wide spectrum of roles, behaviors, and rhetorical strategies that can shape online discourse in both constructive and destructive ways. This work conceptualizes these automated actors as \textbf{Cyber Social Agents} through a taxonomy of archetypes characterized by their operational tactics and rhetorical style. We integrate this taxonomy into an LLM-driven social simulation, where agents communicate and coordinate in a network environment. Using empirically grounded CSA personas, we simulate heterogeneous online societies to study how agent diversity shapes information diffusion and social influence. Our approach bridges the gap between rule-based agent models and LLM-powered simulations with generated agents that are parameterized from empirical data.

==> tablebot.tex <==
\begin{table}[h]
\centering
\caption{Cyber Social Agent Archetypes}
\label{tab:personas}
\begin{tabular}{p{3cm}p{3.5cm}p{6.5cm}}
\toprule
\textbf{Category} & \textbf{Archetype} & \textbf{Primary Function} \\
\midrule
Information & News Bot & Delivers or aggregates timely news updates \\ 
~ & Announcer & Issues scheduled or periodic information releases \\ 
~ & Content Generator & Creates original social media content (novel or synthetically generated) \\ \hline 
Influence & Amplifier & Increases message reach through high frequency shares \\ 
~ & Repeater & Replicates its existing content to reinforce narratives \\ 
~ & Social Influencer & Applies persuasive tactics \\ 
~ & Synchronized & Coordinates with peer agents \\ \hline 
Engagement & Conversational & Sustains dialogue or initiates discussion in threads \\ 
~ & Bridger & Connects distinct communities or network clusters \\ 
~ & Engagement Generator & Evokes emotional responses and drive user interfaces \\ \hline 
Correction & Information Corrector & Detects and counter false information \\ \hline
Disruption & Chaos & Injects randomness or conflict to fragment discourse \\ \hline 
Hybrid & Cyborg & Blends human input with automated posting behavior \\ 
~ & Genre-Specific & Focuses activity within a defined topical domain \\ 
~ & General & Executes broad, non-specialized automated actions \\ 
\bottomrule
\end{tabular}
\end{table}
